Verified Training for Counterfactual Explanation Robustness under Data Shift

Counterfactual explanations (CEs) enhance the interpretability of machine learning models by describing what changes to an input are necessary to change its prediction to a desired class. These explanations are commonly used to guide users' actions, e.g., by describing how a user whose loan application was denied can be approved for a loan in the future. Existing approaches generate CEs by focusing on a single, fixed model, and do not provide any formal guarantees on the CEs' future validity. When models are updated periodically to account for data shift, if the generated CEs are not robust to the shifts, users' actions may no longer have the desired impacts on their predictions. This paper introduces VeriTraCER, an approach that jointly trains a classifier and an explainer to explicitly consider the robustness of the generated CEs to small model shifts. VeriTraCER optimizes over a carefully designed loss function that ensures the verifiable robustness of CEs to local model updates, thus providing deterministic guarantees to CE validity. Our empirical evaluation demonstrates that VeriTraCER generates CEs that (1) are verifiably robust to small model updates and (2) display competitive robustness to state-of-the-art approaches in handling empirical model updates including random initialization, leave-one-out, and distribution shifts.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/old/approach.tex <==
% ---------------------
% section 4.1, deleted text for reference
% ----------------------
\Cref{alg:robust_train} yields a classifier $f$ whose CFXs will be robust to small future changes in the model and a CFX generator $\gen$ that generates robust CFXs.
During each epoch, \cref{alg:robust_train} iteratively optimize the model $f$ and the CFX generator $\gen$ such that the CFXs generated will be $\mult_{f, \x}$-robust. 
First, the generator $\gen$ will generate a set of CFXs $\cfx{\x}_1, \cfx{\x}_2, \ldots, \cfx{\x}_n$ 
% that are robust over $\mult_{f,\x}$ (\cref{eq:rob_cfx_mult}) 
with respect to the classifier $f$ and the training set $D$ (line~3). 
Next, the classifier $f$ can be optimized via $\nabla_{\param{f}} \lossf$ so that each of the generated CFXs $\cfx{\x}_i$ will be $\mult_{f, \x}$-robust (line~4).
At the end of each epoch, the CFX generator $\gen$ can be optimized via $\nabla_{\param{\gen}} \lossgen$ so that it can generate more robust CFXs (line~5).
Note that our approach can train a classifier $f$ with respect to a given CFX generator $\gen$ such that the generated CFXs are $\mult_{f, \x}$-robust as shown in \cref{alg:robust_train_fonly}.

$\lossf$ contains the original CounterNet loss prompting classification accuracy of model $f$ and our proposed RobustCFX loss $\lossrobust$, which measures the robustness of a CFX $\cfx{\x}$ with respect to $\mult_{f,\x}$, which is defined by hyper-parameters $\delta, p$.
For simplicity, we will omit $\delta, p$ from the RobustCFX loss.
$\lossgen$ has three terms. The first two terms are the original CounterNet losses, aiming to minimize proximity and maximize CFX validity, i.e., the generated CFX $\cfx{\x}_i$ should be classified as $1-y_i$ by $f$.
The last term of $\lossgen$ is the RobustCFX loss $\lossrobust$ proposed by our approach.

==> sections/old/definition.tex <==
% Note that \cref{def: multiplicityset} is more expressive than the one defined in \citet{drobustness_inn}.
% \todored{Please see Appendix for a more detailed discussion.}


% \anna{does our code only consider models that have the same prediction on x? (I don't think so because we don't train models on a per-smaple basis and AFAIK there's no robustness check before generating \cf. So, I think we should just remove the x must be robust criteria -- if x isn't robust, then that's OK because they just (presumably) want the opposite pred. so doesn't matter if that's via the \cf{} or not} 
% \yuhao{For the ``ours'' setting, yes, the approach aims to only consider the models that have same prediction on $\x$, but not precisely, since we still need overapproximation. However, for ``IBP'' and ``CROWNIBP'' settings, these approaches do not consider this constraint.}



% \paragraph{Counterfactual explanations}
% \cf{} are commonly used in socially-salient situations, e.g., to explain why an individual's application for a loan was denied. 
% In these situations, \cf{} are also called algorithmic recourse, because they describe how an individual can obtain a different prediction through actionable changes to their feature data. 
% For a binary classifier $f$ and an input $\x$, a \cf{} is another data point $\cfx{\x}$ such that $\cfx{\x}$ is close to the original input $\x$ but receives a different prediction from $f$. 
% To generate such a \cf{} $\cfx{\x}$, existing work~\citep{xxx} \todored{cite} usually minimizes $||\x-\cfx{\x}||_1$ subject to the constraint $f(\cfx{\x}) = 1 - f(\x)$.
% A \cf{} $\cfx{\x}$ is \emph{valid} if $f(\cfx{\x}) = 1 - f(\x)$.
% The $l_1$ distance between a \cf{} and the original input is call \emph{proximity}.
% Additional constraints (e.g., not changing immutable features like race or sex) can be placed on the \cf{} generation process, e.g., by using a custom distance metric that heavily penalizes changing those features. Our approach is compatible with those modifications, but for simplicity we will assume that a $l_1$ distance metric is appropriate.

% We denote a \cf{} generation algorithm as a function $\gen$, which takes inputs as the classifier $f$ and the original input $\x$, and outputs a \cf{} $\cfx{\x}=\gen(f, \x)$.

% Counterfactual explanations are commonly used in socially-salient situations, e.g., to explain why a user's application for a loan was denied. 
% In these situations, a \cf{} is also called algorithmic recourse. 
% It is desirable for algorithmic recourse to be actionable (e.g., $\x$ and $\cfx{\x}$ should have the same gender, race, etc, but may vary on mutable features like salary). 





% \yuhao{copied from the grant proposal, need to redesign the example}
% \anna{removing for space, we give intuition of why \cf{} robustness matters in the intro}
% \begin{example}[\cf{} robustness]\label{ex:cfx_shift}
%     Suppose a student applies to an internship but is rejected. The rejection may be accompanied by a counterfactual explanation, e.g., ``you would have been hired if your GPA were 0.2 points higher and you had taken 1 additional upper-level course.'' 
%     The student decides to re-apply for an internship the following summer, and focuses on improving their GPA while taking another upper-level class. 
%     If the company updates their model in the next hiring cycle, the features GPA and number of upper-level electives might become less relevant, thus making the student's effort ineffective!
% \end{example}



% \anna{if we adopt my comment below, add: Notably, we do not require that $\x$ be robust over $\mult$. Intuitively, this is because we assume that $\x$ will, in parallel with any model updates, morph into $\x'$, thus making the prediction of $\x$ on the new model irrelevant. }

% In this paper, we assume that the old model $f$ will be slightly modified on the new data to obtain a new model $\rs$. 
% There are multiple ways to obtain such a slightly-modified model.
% For example, fine-tuning is a process of taking an existing model and performing a small number of additional training epochs on the new data.
% Another way is to retrain from scratch while adding l2 regularization such that all the model parameters will be bounded within a small range.

% For instance, consider a linear model $f(\x)=\mathbb{1}\{W_f\x+b_f>0\}$ with $W_f=(1,-1)$ and $b_f=-2$. If use $\delta=2$ and the $l_{\infty}$ norm, we have $\mult_{f,\x}=\{\rs\mid f(\x)=\rs(\x)\land \|W_f-W_{\rs}\|_{\infty}\leq 2 \land \|b_f - b_{\rs}\|_{\infty}\leq 2\}$. \yuhao{I feel this example does not help. Maybe we should point to Figure~\ref{fig:example1_plots}} \anna{not sure if there's a good way to comment on fig. 1 here w/o just reiterating ex. 1. So commenting this para out}

% \begin{example}
%     Consider a linear model with $W_f = (1, -1), b_f = -2$ and $f(\x) = \mathds{1}\{W_f\x + b_f > 0\}$.
%     Given an original input $\x = (4, 1)$, we define the multiplicity set $\mult_{f,\x} = \{ \rs \mid f(\x) = \rs(\x) \wedge \|W_{f} - W_{\rs}\|_{\infty} \le 2  \wedge \|b_{f} - b_{\rs}\|_{\infty} \le 2\}$ with $p=\infty$ and $\delta=2$.

%     A model $f_1$ with $W_{f_1} = (3, 1), b_{f_1}=-4$ is in $\mult_{f,\x}$, while $f_2$ with $W_{f_2} = (3, 1), b_{f_2}=-5$ or $f_3$ with $W_{f_3} = (-1, -1), b_{f_3}=-2$ are not because $\|b_{f} - b_{f_2}\|_\infty > 2$ and $f(\x) \neq f_3(\x)$. 
% \end{example}

==> sections/old/experiments.tex <==
% \subsection{Main Results}

% We compare our approach with other approaches:
% \begin{itemize}
%     \item \textbf{Standard training + [Wachter/Proto]} We train a model $M_{ori}$ using standard training. Then generate CFXs $X'$ using Wachter/Proto. Finally, train other models $M_{shift}$ under dataset shifts using standard training and evaluate $X'$ on $M_{shift}$. 
%     \item \textbf{Our approach + [Wachter/Proto]} We train a model $M_{ori}$ using our approach that takes a third-party CFX tool, e.g., Wachter or Proto. Then generate CFXs $X'$ using Wachter/Proto. Finally, train other models $M_{shift}$ under dataset shifts using our approach and evaluate $X'$ on $M_{shift}$. 
%     \item \textbf{Standard training + [ROAR/T-Rex/SNS/INN]} This setting is similar to the first setting, but we use robust generation methods to generate CFX instead of standard CFX generation tool.
%     \item \textbf{Our approach + [ROAR/T-Rex/SNS/INN]} This setting is similar to the second setting, but our approach uses robust generation methods during training and we use the corresponding robust CFX generation method to generate CFX.
%     \item \textbf{CounterNet} We train a model $M_{ori}$ using CounterNet. Then generate CFXs $X'$ using CounterNet. Finally, train other models $M_{shift}$ under dataset shifts using CounterNet and evaluate $X'$ on $M_{shift}$. 
%     \item \textbf{Our approach + CounterNet} We train a model $M_{ori}$ using our approach + CounterNet. Then generate CFXs $X'$ using CounterNet. Finally, train other models $M_{shift}$ under dataset shifts using Our approach + CounterNet and evaluate $X'$ on $M_{shift}$. 
% \end{itemize}

% Metrics: model test accuracy. validity/ robustness/ proximity/ sparsity/ distance-to-manifold of CFX.
% The robustness of CFX is generated by MILP solver (for ReLU neural networks), or by our verification approach (for any neural networks).
